Tackling Shortcut Learning in Deep Neural Networks: An Iterative Approach with Interpretable Models

We use concept-based interpretable models to mitigate shortcut learning. Existing methods lack interpretability. Beginning with a Blackbox, we iteratively carve out a mixture of interpretable experts (MoIE) and a residual network. Each expert explains a subset of data using First Order Logic (FOL). While explaining a sample, the FOL from biased BB-derived MoIE detects the shortcut effectively. Finetuning the BB with Metadata Normalization (MDN) eliminates the shortcut. The FOLs from the finetuned-BB-derived MoIE verify the elimination of the shortcut. Our experiments show that MoIE does not hurt the accuracy of the original BB and eliminates shortcuts effectively.

==> Sections/concept_importance_v1.tex <==
\cref{fig:valid_concepts}(a-b) shows that MoIE achieves high completeness scores~\cite{yeh2019concept} (\cref{app:completeness} for details) for the varying number of concepts than the baselines. Also ~\cref{fig:valid_concepts}(c-d) illustrates MoIE records more the drop in accuracy than the baselines when we set the values of the significant concepts zeroes. Recall, $g$ utilizes E-LEN~\cite{barbiero2022entropy}, associating each concept with an attention weight after training. A concept with high attention weight implies its high predictive significance.
As MoIE deploys multiple experts for different subsets of data, they identify highly significant concepts, resulting in higher completeness scores and more accuracy drop. Refer to~\cref{app:qual} for comparing FOLs by MoIE and the baselines. 

